xMOD: Cross-Modal Distillation for 2D/3D Multi-Object Discovery from 2D motion

Object discovery, which refers to the task of localizing objects without human annotations, has gained significant attention in 2D image analysis. However, despite this growing interest, it remains under-explored in 3D data, where approaches rely exclusively on 3D motion, despite its several challenges. In this paper, we present a novel framework that leverages advances in 2D object discovery which are based on 2D motion to exploit the advantages of such motion cues being more flexible and generalizable and to bridge the gap between 2D and 3D modalities. Our primary contributions are twofold: (i) we introduce DIOD-3D, the first baseline for multi-object discovery in 3D data using 2D motion, incorporating scene completion as an auxiliary task to enable dense object localization from sparse input data; (ii) we develop xMOD, a cross-modal training framework that integrates 2D and 3D data while always using 2D motion cues. xMOD employs a teacher-student training paradigm across the two modalities to mitigate confirmation bias by leveraging the domain gap. During inference, the model supports both RGB-only and point cloud-only inputs. Additionally, we propose a late-fusion technique tailored to our pipeline that further enhances performance when both modalities are available at inference. We evaluate our approach extensively on synthetic (TRIP-PD) and challenging real-world datasets (KITTI and Waymo). Notably, our approach yields a substantial performance improvement compared with the 2D object discovery state-of-the-art on all datasets with gains ranging from +8.7 to +15.1 in F1@50 score. The code is available at https://github.com/CEA-LIST/xMOD

==> sec/subsections/fig_sphe_vs_front.tex <==
\begin{figure*}[tbp]
    \centering
    \begin{subfigure}{0.24\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{figures/front_3d.png}
        \caption{Front-view projection}
        \label{fig:graph_losssub1}
    \end{subfigure}
    % \hfill
    \begin{subfigure}{0.24\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{figures/mask_orig.png}
        \caption{Original motion mask}
        \label{fig:graph_losssub3}
    \end{subfigure}
     \hfill
    \begin{subfigure}{0.24\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{figures/sphe_3d.png}
        \caption{Spherical projection}
        \label{fig:graph_lossub2}
    \end{subfigure}
    % \hfill
    \begin{subfigure}{0.24\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{figures/mask_sphe.png}
        \caption{Projected motion mask}
        \label{fig:graph_lossub4}
    \end{subfigure}
    \caption{Spherical projection creates denser LiDAR data maps but results in partial object representation in 2D-3D cross-modal tasks. Front-view projection is preferred for 3D object discovery to avoid these issues.}
    \label{fig:sphe_vs_front}
\end{figure*}

==> sec/subsections/overview.tex <==

\svgpath{{figures}}
\begin{figure*}[tb]
  \centering
\includegraphics[trim={0 0 3cm 0},clip,width=0.9\linewidth]{figures/cross_modal_v19.pdf}
%   \includesvg[width=0.8\textwidth]{cross_modal_v18.svg}
  
   \caption{\textbf{Overview of the proposed approach}. \textbf{i) DIOD-3D}. At each iteration, a sequence front-view projections of point clouds is passed to the 3D teacher and student models. Attention maps from the teacher model are presented as targets to the student model through $L^{dist}_{3D\rightarrow3D}$.  An MSE objective is employed to predict the original scene from input with missing data, enabling 3D scene completion as an auxiliary task for 3D object discovery. \textbf{ii) Cross-modal distillation (xMOD)}. Alongside the 3D branch, sequences of RGB images are forwarded to the 2D teacher and student models. $L^{dist}_{2D\rightarrow3D}$ means pseudo-labels from the 2D teacher model are aligned with the 3D student input and used for its supervision; $L^{dist}_{3D\rightarrow2D}$ works similarly for 3D to 2D pseudo-labeling. Motion pseudo-labels $\mathcal{M}_{2D}$ and $\mathcal{M}_{3D}$ are used for regularization, with $\mathcal{M}_{3D}$ being the 2D motion segments with corresponding 3D points. We omit representing 2D reconstruction and 3D completion task for simplification.}
   \label{fig:overview}
\end{figure*}
